An Enhanced Model for Stochastic Coordination

Applications developed over the cloud coordinate several, often anonymous, computational resources, distributed over different execution nodes, within flexible architectures. Coordination models able to represent quantitative data provide a powerful basis for their analysis and validation. This paper extends IMCreo, a semantic model for Stochastic reo based on interactive Markov chains, to enhance its scalability, by regarding each channel and node, as well as interface components, as independent stochastic processes that may (or may not) synchronise with the rest of the coordination circuit.

==> eptcsdata.tex <==
\providecommand{\firstpage}{35}
\providecommand{\publicationstatus}{R. Behjati and A. Elmokashfi (Eds.): Workshop on\\
Formal Methods for and on the Cloud (iFMCloud'16)\\
EPTCS 228, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.228.5}{10.4204/EPTCS.228.5}}

